Share, Collaborate, Benchmark: Advancing Travel Demand Research through rigorous open-source collaboration

This research foregrounds general practices in travel demand research, emphasizing the need to change our ways. A critical barrier preventing travel demand literature from effectively informing policy is the volume of publications without clear, consolidated benchmarks, making it difficult for researchers and policymakers to gather insights and use models to guide decision-making. By emphasizing reproducibility and open collaboration, we aim to enhance the reliability and policy relevance of travel demand research. We present a collaborative infrastructure for transit demand prediction models, focusing on their performance during highly dynamic conditions like the COVID-19 pandemic. Drawing from over 300 published papers, we develop an open-source infrastructure with five common methodologies and assess their performance under stable and dynamic conditions. We found that the prediction error for the LSTM deep learning approach stabilized at a mean arctangent absolute percentage error (MAAPE) of about 0.12 within 1.5 months, whereas other models continued to exhibit higher error rates even a year into the pandemic. If research practices had prioritized reproducibility before the COVID-19 pandemic, transit agencies would have had clearer guidance on the best forecasting methods and quickly identified those best suited for pandemic conditions to inform operations in response to changes in transit demand. The aim of this open-source codebase is to lower the barrier for other researchers to replicate, reproduce models and build upon findings. We encourage researchers to test their own modeling approaches on this benchmarking platform, challenge the analyses conducted in this paper, and develop model specifications that can outperform those evaluated here. Further, collaborative research approaches must be expanded across travel demand modeling if we wish to impact policy and planning.

==> sections/01_intro.tex <==
\section{Introduction}

The motivation behind dynamic routing is to be responsive to real-time demand and improve transit services and reliability. Short-term demand prediction supports the decision-making process in dynamic routing by providing ridership forecasts to allow the allocation of resources ahead of time. In a highly dynamic situation (e.g., a situation that is both unexpected and uncertain), these decisions become more relevant. As demand changes drastically, public transit agencies need to adjust their fleet operations to meet the new demand needs. Examples of highly dynamic conditions are the coronavirus disease 2019 (COVID-19) pandemic and the effects of long-term protests. The induced lockdowns during the COVID-19 pandemic resulted in drastic changes in travel demand, and the duration of these changes was (and still is) uncertain because of the novelty of the virus. Thus, many transit agencies responded by reducing and modifying transit services. While most protests might be foreseeable in the short term, their aftermath is not. Protests might last weeks or months, potentially affecting  the public transit infrastructure and forcing temporary station closures and transit services modifications. Despite the impact of these scenarios, the literature on short-term ridership prediction methods has been limited to short, stable time frames and a few stations in one geographical area. While we hypothesize that these models may lose predictive power in highly dynamic conditions, some may still provide valuable guidance to transit agencies, supporting decision-making in environments with limited information. However, how these models perform in highly dynamic conditions has not been studied, nor has their performance been systematically compared.

The ability to generate accurate and reliable results in highly dynamic conditions hinges on our capacity to compare models swiftly and draw robust conclusions that address the situation at hand. However, over the last decade, the literature on short-term ridership prediction methods has grown exponentially, encompassing diverse approaches that make it challenging for individual researchers to keep pace, reproduce models, and conduct meaningful comparisons in time to be useful in highly dynamic conditions(traditional research timeline no longer seems to support the fast evolving conditions of highly dynamic conditions).  Code and data are often unavailable, requiring researchers to re-implement methods, which leads to potentially inconsistent results making replication difficult. Additionally, benchmarks typically include a small subset of models, limited by the time and resources available to the researchers. These practices severely hinder the research community's ability to identify relevant literature, consuming valuable time and compromising timely responses to highly dynamic conditions.This scenario demands for a concentrated action to create a standardized platform for implementing and benchmarking the various models, facilitating collaborative efforts to generate collective wisdom for use when it is most needed.

The objectives of this research are to facilitate accurate and reliable comparison of short-term ridership prediction models and to compare and assess the performance of state-of-the-art models in highly dynamic conditions. To achieve these objectives, we propose an open-source codebase containing five widely used models, including two statistical models, autoregressive integrated moving average (ARIMA)  and seasonal ARIMA (SARIMA), and three deep learning models, the multilayer perceptron (MLP), convolutional neural networks (CNN), and the long-short-term memory network (LSTM). These methods are substantially different in how they structure and process time series data and are widely used for short-term ridership prediction models and other time series applications. 

We use more than five years of data from the bus rapid transit (BRT) system in Bogot\'{a}, Colombia, which is publicly available and can be used by other researchers. This dataset contains two highly dynamic conditions: a month-long protest in November and December 2019 and the COVID-19 pandemic since March 2020. Given the sudden demand changes with highly dynamic conditions and the complex spatiotemporal correlation of transit demand, we also tested the performance of the models with an “adaptive training” and “multi-output” model design. The adaptive training model retrains the model as new information becomes available, which can improve model performance in highly dynamic conditions. The multi-output model aims to consolidate the prediction of individual stations into one model, capturing possible spatial and temporal correlations across stations. 

The contributions of this research are two-fold: first, to create an open-source codebase infrastructure using a publicly available dataset to produce standard, reliable, and statistically rigorous benchmarks for short-term ridership prediction models and to employ this infrastructure to compare and assess the performances of state-of-the-art models in highly dynamic conditions and different model designs.

The remainder of the paper is organized as follows. Section 2 summarizes the relevant literature for short-term public transit demand forecasting. Next, Section 3 explains the meta-analysis methodology, including appropriate research methods and modeling strategies. Then, Section 4 presents the meta-analysis results, and Section 5 concludes with the discussion and conclusion. 


to add to lit review: 

statistical models \citep{Milenkovic2018, Ding2017, Sun2014}, machine learning \citep{Sun2015, Li2017, Ding2016, Toque2018, Dai2018,  Chen2011}, deep learning \citep{Tsai2009,Wei2012,9141203,Liu2019,8951085,Borovykh2017ConditionalTS,cho-etal-2014-properties,6795963, ijgi8060243, ZHANG2021102928, Bai2017}, Bayesian approaches \citep{Roos2017}, optimization \citep{Glisovic2016, Xie2020, Yuan2019}, gray theory \citep{Jia2016, Wang2019}, gravity models \citep{Shen2020}, Kalman filtering \citep{Zhang2011, Jiao2016} and even combinations of these approaches \citep{Jing2021,MA2014148,Zhang2022,Zhang2019}.

==> sections/intro_reframing.tex <==
Share, Collaborate, Forecast: Advancing Travel Demand Research through rigorous open-source collaboration. 
Abstract 
This paper presents a critical examination of the traditional methodologies used in travel demand research, highlighting their limitations in adapting to rapid socio-economic changes, such as pandemics and shifts in work culture. Traditional travel demand models often struggle to keep pace with abrupt changes in transit patterns, leading to outdated or ineffective policy decisions. To address these challenges, we advocate for a fundamental shift in research practices toward more agile and collaborative approaches. THE SHIFT IS MAJOR, NEED TO CHANGE OUR WAY OF THINKING AND NORMS. HERE WE MOTIVATE WITH ONE SPECIFIC LITERATURE AND DEMONSTRATE HOW IT CAN BE DONE DIFFERENTLY. Specifically, we propose (we propose one example) the development of an open-source platform that facilitates the sharing of methodologies and data. This platform aims to enhance the replicability and benchmarking of research by providing researchers with access to a collective pool of rigorously tested models. This approach is exemplified through a meta-analysis of transit demand ridership prediction models, focusing on their performance during highly dynamic conditions. Our study includes a variety of methodologies ranging from statistical models to deep learning, assessing their adaptability to sudden changes in transit demand. The findings underscore the necessity for research practices that can swiftly respond to changing conditions, ensuring that travel demand models remain relevant and practical for decision-making. The contributions of this research are twofold: the creation of a collaborative, open-source codebase to apply diverse modeling approaches to real-world data, and the execution of comparative analyses that highlight the strengths and weaknesses of existing models under varying scenarios.

Introduction 

In an era marked by rapid technological, cultural, social, and environmental changes that drastically impact travel demand, the current research practices in travel demand research appear increasingly misaligned with reality. Traditional models, although advanced, often fail to capture the abrupt shifts in travel patterns that now characterize our dynamic socio-economic environment, raising doubts about their long-term predictive accuracy. Typically, research has focused on modeling new behavior trends, adapting to new datasets, and considering technological adoption, which has resulted in models that respond to specific changes but rarely undergo comparative performance analysis. This lack of comparative analysis impedes the development of collective wisdom. The travel demand modeling publication process incentivizes strong claims of advantages and uniqueness and underemphasizes reproducibility and comparability. Therefore from this literature it is not possible to answer critical questions for scientific progress: What are the most promising approaches? Which are perhaps good ideas, but can be left aside? Are the findings robust? Are they honest? Such a disconnect not only undermines research's ability to provide timely, actionable insights. [examples from other fields… hurricane forecasting, machine learning and vision, psychology.] This paper critiques the existing methodologies in travel demand research for their lack of flexibility and agility and and demonstrate a different approach to … proposes a novel approach to reorient research practices.

Current research practices are challenged by their slow and inflexible nature, difficulties in replicability and benchmarking, and a trend of exponential publication growth—all of which hinder our ability to generate collective wisdom. Traditional research is slow and inflexible. We normally face a new issue, we need to make the model sensitive to it, so we go and collect survey data, and then we estimate the model, we might need to come up with a new model structure to fully explain more and more, and by the time that the research is publish, preferences might have already change, or even new alternatives are already in the horizon and the model might no longer support the decision-making process. While many papers provide sufficient methodological details to replicate the method, but the implementation is rarely shared, leaving it to other researchers to re-implement from scratch which’s can leads to potentially inconsistent results making replication difficult. On many occasions, dataset is not share either, therefore, to warranty fully replicability is almost impossible, and even impractical. Additionally, in the last decades, there has been a proliferation of research studies. This is especially true when trying to benchmark model performance with existing models in the literature. As mentioned before, replicability of methods is difficult, and combined with multiple methods, it becomes impractical. As a result, benchmarks typically include a small subset of models, limited by the time and resources available to the researchers, making the comparison incomplete and fragmented.

Slow and inflexible research, lack of replicability and overproduction of research not only dilutes the impact of individual studies, but also makes it harder for researchers to identify relevant research in a timely manner to provide the best information for the policy makers the ability of researchers to discern and deploy actionable insights in a timely manner in a world that is constantly changing. Keep asking questions on how to model a new behavior, a new technology, a new adoption is not enough. Before revisiting and rethinking the assumption or formulations of our travel demand models, we need to revisit and rethink how we, as a research community, are performing research in a way that is methodological, rigorous and impactful, and that generates collective wisdom.  

Therefore, the objective of this research is to demonstrate one aspect of how research in travel demand can be done differently. We advocate for the creation of an open-source platform designed to foster collaboration within the research community. By facilitating consistent benchmarking and comparative analysis of predictive models across diverse scenarios, this platform will not only streamline the adaptation and implementation of models but also ensure they meet established standards without the need for complete redevelopment. As a result, it will simplify and streamline access to pre-implemented, easy-to-use models. Serving as a collaborative hub, the platform will empower researchers to both contribute to and utilize a collective pool of rigorously tested models, thereby accelerating the process of model evaluation and refinement. 

In this research, we focus on the transit demand ridership prediction problem. In the last few years, there has been a large number of studies proposing new transit demand models, which different approaches varying from statistical models \citep{Milenkovic2018, Ding2017, Sun2014}, machine learning \citep{Sun2015, Li2017, Ding2016, Toque2018, Dai2018,  Chen2011}, deep learning \citep{Tsai2009,Wei2012,9141203,Liu2019,8951085,Borovykh2017,cho-etal-2014-properties,6795963, ijgi8060243, ZHANG2021102928, Bai2017}, Bayesian approaches \citep{Roos2017}, optimization \citep{Glisovic2016, Xie2020, Yuan2019}, gray theory \citep{Jia2016, Wang2019}, gravity models \citep{Shen2020}, Kalman filtering \citep{Zhang2011, Jiao2016} and even combinations of these approaches \citep{Jing2021,MA2014148,Zhang2022,Zhang2019}. As stated above, code and data are often not shared making replicability difficult resulting in benchmarks that only compare a small subset of methods, making the comparison incomplete and fragmented. In the light of the COVID-19 pandemic, transit agencies were forced make rapid adjustments without the data-driven guidance typically provided by predictive models. Some of these adjustments were made equally across cities, not considering that certain communities might still need transit more than others, (https://www.sciencedirect.com/science/article/pii/S1361920922002619). While the hypothesis that models during highly dynamic conditions loss predictive power, it is also true that we could have asked questions like among the existing models, which one adapt faster to the current condition. While we hypothesize that these models may lose predictive power in highly dynamic conditions, some may still provide valuable guidance to transit agencies, supporting decision-making in environments with limited information. However, how these models perform in highly dynamic conditions has not been studied, nor has their performance been systematically compared, even under stable conditions. 

The contributions of this research are twofold: firstly, we showcase/demonstrate that the creation of an open-source codebase that facilitates the application of statistical and deep learning models to real-world data sets; and secondly, the use of this infrastructure to conduct rigorous, comparative analyses of model performances across various scenarios. This approach not only aims to streamline the model comparison process but also to cultivate a repository of readily deployable, empirically tested solutions that can adapt to and inform rapidly evolving transit demand.

The remainder of the paper is organized as follows. Section 2 summarizes the relevant literature for short-term public transit demand forecasting. Next, Section 3 explains the meta-analysis methodology, including appropriate research methods and modeling strategies. Then, Section 4 presents the meta-analysis results, and Section 5 concludes with the discussion and conclusion, and a thought exercise of where OUR knowledge would be if we lean into practices like this. 

